Abstracting Noisy Robot Programs

Abstraction is a commonly used process to represent some low-level system by a more coarse specification with the goal to omit unnecessary details while preserving important aspects. While recent work on abstraction in the situation calculus has focused on non-probabilistic domains, we describe an approach to abstraction of probabilistic and dynamic systems. Based on a variant of the situation calculus with probabilistic belief, we define a notion of bisimulation that allows to abstract a detailed probabilistic basic action theory with noisy actuators and sensors by a possibly non-stochastic basic action theory. By doing so, we obtain abstract Golog programs that omit unnecessary details and which can be translated back to a detailed program for actual execution. This simplifies the implementation of noisy robot programs, opens up the possibility of using non-stochastic reasoning methods (e.g., planning) on probabilistic problems, and provides domain descriptions that are more easily understandable and explainable.

==> rwth-colors.tex <==
\definecolor{rwth-blue}{cmyk}{1,.5,0,0}
\definecolor{rwth-lblue}{cmyk}{0.75,0.38,0,0}
\definecolor{rwth-llblue}{cmyk}{0.45,0.14,0,0}
%\definecolor{rwth-llblue}{RGB}{142,186,229}
\definecolor{rwth-lllblue}{cmyk}{0.23,0.07,0,0}
\definecolor{rwth-llllblue}{cmyk}{0.09,0.03,0,0}
%\colorlet{rwth-lblue}{rwth-blue!75}
%\colorlet{rwth-llblue}{rwth-blue!50}
%\colorlet{rwth-lllblue}{rwth-blue!25}
%\colorlet{rwth-llllblue}{rwth-blue!10}

\definecolor{rwth-black}{cmyk}{0,0,0,1}
\colorlet{rwth-lblack}{rwth-black!75}
\colorlet{rwth-llblack}{rwth-black!50}
\colorlet{rwth-lllblack}{rwth-black!25}
\colorlet{rwth-llllblack}{rwth-black!10}

\definecolor{rwth-magenta}{cmyk}{0,1,.25,0}
\colorlet{rwth-lmagenta}{rwth-magenta!75}
\colorlet{rwth-llmagenta}{rwth-magenta!50}
\colorlet{rwth-lllmagenta}{rwth-magenta!25}
\colorlet{rwth-llllmagenta}{rwth-magenta!10}

\definecolor{rwth-yellow}{cmyk}{0,0,1,0}
\colorlet{rwth-lyellow}{rwth-yellow!75}
\colorlet{rwth-llyellow}{rwth-yellow!50}
\colorlet{rwth-lllyellow}{rwth-yellow!25}
\colorlet{rwth-llllyellow}{rwth-yellow!10}

\definecolor{rwth-petrol}{cmyk}{1,0.3,0.5,0.3}
\colorlet{rwth-lpetrol}{rwth-petrol!75}
\colorlet{rwth-llpetrol}{rwth-petrol!50}
\colorlet{rwth-lllpetrol}{rwth-petrol!25}
\colorlet{rwth-llllpetrol}{rwth-petrol!10}

\definecolor{rwth-turquoise}{cmyk}{1,0,0.4,0}
\colorlet{rwth-lturquoise}{rwth-turquoise!75}
\colorlet{rwth-llturquoise}{rwth-turquoise!50}
\colorlet{rwth-lllturquoise}{rwth-turquoise!25}
\colorlet{rwth-llllturquoise}{rwth-turquoise!10}

\definecolor{rwth-green}{cmyk}{.7,0,1,0}
\colorlet{rwth-lgreen}{rwth-green!75}
\colorlet{rwth-llgreen}{rwth-green!50}
\colorlet{rwth-lllgreen}{rwth-green!25}
\colorlet{rwth-llllgreen}{rwth-green!10}

\definecolor{rwth-grass}{cmyk}{.35,0,1,0}
\colorlet{rwth-lgrass}{rwth-grass!75}
\colorlet{rwth-llgrass}{rwth-grass!50}
\colorlet{rwth-lllgrass}{rwth-grass!25}
\colorlet{rwth-llllgrass}{rwth-grass!10}

\definecolor{rwth-orange}{cmyk}{0,.4,1,0}
\colorlet{rwth-lorange}{rwth-orange!75}
\colorlet{rwth-llorange}{rwth-orange!50}
\colorlet{rwth-lllorange}{rwth-orange!25}
\colorlet{rwth-llllorange}{rwth-orange!10}

\definecolor{rwth-red}{cmyk}{.15,1,1,0}
\colorlet{rwth-lred}{rwth-red!75}
\colorlet{rwth-llred}{rwth-red!50}
\colorlet{rwth-lllred}{rwth-red!25}
\colorlet{rwth-llllred}{rwth-red!10}

\definecolor{rwth-burgundy}{cmyk}{0.25,1,0.7,0.2}
\colorlet{rwth-lburgundy}{rwth-burgundy!75}
\colorlet{rwth-llburgundy}{rwth-burgundy!50}
\colorlet{rwth-lllburgundy}{rwth-burgundy!25}
\colorlet{rwth-llllburgundy}{rwth-burgundy!10}

\definecolor{rwth-violet}{cmyk}{0.7,1,0.35,0.15}
\colorlet{rwth-lviolet}{rwth-violet!75}
\colorlet{rwth-llviolet}{rwth-violet!50}
\colorlet{rwth-lllviolet}{rwth-violet!25}
\colorlet{rwth-llllviolet}{rwth-violet!10}

\definecolor{rwth-purple}{cmyk}{0.6,0.6,0,0}
\colorlet{rwth-lpurple}{rwth-purple!75}
\colorlet{rwth-llpurple}{rwth-purple!50}
\colorlet{rwth-lllpurple}{rwth-purple!25}
\colorlet{rwth-llllpurple}{rwth-purple!10}

\definecolor{rwth-cyan}{cmyk}{1,0,.4,0}\colorlet{rwth-lcyan}{rwth-cyan!50}\colorlet{rwth-llcyan}{rwth-cyan!25}
\definecolor{rwth-teal}{cmyk}{1,.3,.5,.3}\colorlet{rwth-lteal}{rwth-teal!50}\colorlet{rwth-llteal}{rwth-teal!25}
\definecolor{rwth-silver}{cmyk}{.39,.31,.32,.14}
\definecolor{rwth-gold}{cmyk}{.35,.46,.7,.35}

\def\blue#1{\textcolor{rwth-blue}{#1}}\renewcommand{\blue}[2][100]{\textcolor{rwth-blue!#1}{#2}}
\def\violet#1{\textcolor{rwth-violet}{#1}}\renewcommand{\violet}[2][100]{\textcolor{rwth-violet!#1}{#2}}
\def\purple#1{\textcolor{rwth-purple}{#1}}\renewcommand{\purple}[2][100]{\textcolor{rwth-purple!#1}{#2}}
\def\carmine#1{\textcolor{rwth-carmine}{#1}}\renewcommand{\carmine}[2][100]{\textcolor{rwth-carmine!#1}{#2}}
\def\red#1{\textcolor{rwth-red}{#1}}\renewcommand{\red}[2][100]{\textcolor{rwth-red!#1}{#2}}
\def\magenta#1{\textcolor{rwth-magenta}{#1}}\renewcommand{\magenta}[2][100]{\textcolor{rwth-magenta!#1}{#2}}
\def\orange#1{\textcolor{rwth-orange}{#1}}\renewcommand{\orange}[2][100]{\textcolor{rwth-orange!#1}{#2}}
\def\yellow#1{\textcolor{rwth-yellow}{#1}}\renewcommand{\yellow}[2][100]{\textcolor{rwth-yellow!#1}{#2}}
\def\grass#1{\textcolor{rwth-grass}{#1}}\renewcommand{\grass}[2][100]{\textcolor{rwth-grass!#1}{#2}}
\def\green#1{\textcolor{rwth-green}{#1}}\renewcommand{\green}[2][100]{\textcolor{rwth-green!#1}{#2}}
\def\cyan#1{\textcolor{rwth-cyan}{#1}}\renewcommand{\cyan}[2][100]{\textcolor{rwth-cyan!#1}{#2}}
\def\teal#1{\textcolor{rwth-teal}{#1}}\renewcommand{\teal}[2][100]{\textcolor{rwth-teal!#1}{#2}}
\def\silver#1{\textcolor{rwth-silver}{#1}}\renewcommand{\silver}[2][100]{\textcolor{rwth-silver!#1}{#2}}
\def\gold#1{\textcolor{rwth-gold}{#1}}\renewcommand{\gold}[2][100]{\textcolor{rwth-gold!#1}{#2}}
\def\black#1{\textcolor{black}{#1}}\renewcommand{\black}[2][100]{\textcolor{black!#1}{#2}}
\def\white#1{\textcolor{white}{#1}}

